Use of recommendation models to provide support to dyslexic students

Dyslexia is the most widespread specific learning disorder and significantly impair different cognitive domains. This, in turn, negatively affects dyslexic students during their learning path. Therefore, specific support must be given to these students. In addition, such a support must be highly personalized, since the problems generated by the disorder can be very different from one to another. In this work, we explored the possibility of using AI to suggest the most suitable supporting tools for dyslexic students, so as to provide a targeted help that can be of real utility. To do this, we relied on recommendation algorithms, which are a branch of machine learning, that aim to detect personal preferences and provide the most suitable suggestions. We hence implemented and trained three collaborative-filtering recommendation models, namely an item-based, a user-based and a weighted-hybrid model, and studied their performance on a large database of 1237 students' information, collected with a self-evaluating questionnaire regarding all the most used supporting strategies and digital tools. Each recommendation model was tested with three different similarity metrics, namely Pearson correlation, Euclidean distance and Cosine similarity. The obtained results showed that a recommendation system is highly effective in suggesting the optimal help tools/strategies for everyone. This demonstrates that the proposed approach is successful and can be used as a new and effective methodology to support students with dyslexia.

==> tables.tex <==
%Tables file which contains all the tables presented during the paper
% Table 1
\begin{table}[b!]
\centering
\begin{adjustbox}{width=\textwidth}
\caption{ Brief overview of ML studies aimed at helping students with and without learning difficulties during their academic education. The acronyms in the table refer to different ML models. In particular, NN: Neural network, OCR: object-character recognition, SVM: Suppor Vector Machine, k-NN: k-Nearest Neighbors, LR: Logistic Regression, RF: Random forest}
\label{tab:table_references}
\begin{tabular}{lll}
\hline
\multicolumn{1}{|l}{Reference}                  & Type of ML                                                   & \multicolumn{1}{l|}{Description}                                                                                                                                                                            \\ \hline
\citep{hamid2015computer} & Hidden Markov & \begin{tabular}[c]{@{}l@{}}ML tracks children's mistakes \\
in phonology,speling, reading and writing\end{tabular} \\ \hline
\citep{hoic2015recommender}    & CB, CF, KB                                                   & \begin{tabular}[c]{@{}l@{}}RS systems were combined with\\ Web applications in order to help teachers \\ in design courses and students to choose \\ the activities to integrate in their learning path\end{tabular} \\ \hline
\citep{rodriguez2015student}   & CB, CF, KB                                                   & \begin{tabular}[c]{@{}l@{}}RS systems used to recommend learning \\ objects to student with similar learning styles\end{tabular}                                                                             \\ \hline
\citep{sergis2015enhancing}      & CF                                                           & \begin{tabular}[c]{@{}l@{}}RS is used to suggest, to teachers, new resources\\ to enhance their teaching practices\end{tabular}                                                                              \\ \hline
\citep{bourkoukou2016learning} & CF                                                           & \begin{tabular}[c]{@{}l@{}}RS used to select the best learning path based\\ on the learning style of each user\end{tabular}                                                                                  \\ \hline
\citep{meryem2016toward}       & Hybrid RS                                                    & \begin{tabular}[c]{@{}l@{}}RS aimed at helping the students in choosing their\\ career path\end{tabular}                                                                                                     \\ \hline
\citep{rajapakse2018alexza} & OCR and NN & \begin{tabular}[c]{@{}l@{}}OCR and NN used to support students while \\ reading difficult words\end{tabular} \\ \hline   
\citep{thelijjagoda2019hope} & SVM & \begin{tabular}[c]{@{}l@{}}SVM used to change the difficulty of video-games \\ and exercises.The students report improvements in \\ their skills and are more engaged in learning \end{tabular}                                                                                    \\ \hline
\citep{pan2020multiview}       & NN                                                           & \begin{tabular}[c]{@{}l@{}}Used NN to recommend courses to students and\\ identify those with learning risks\end{tabular}                                                                                    \\ \hline
\citep{suganya2020subjective}  & SVM                                                          & \begin{tabular}[c]{@{}l@{}}ML used to predict students performance and\\ to indicate directions for improvement\end{tabular}                                                                                 \\ \hline
\citep{zingoni2024machine}     & \begin{tabular}[c]{@{}l@{}}SVM, k-NN, \\ LR, RF\end{tabular} & \begin{tabular}[c]{@{}l@{}}ML models used to suggest the best digital\\ tools and learning strategies to dyslexic students\end{tabular}                                                                      \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


%Table 2
\begin{table*}
\centering
\begin{adjustbox}{width=\textwidth}
\caption{Difficulties (P), support tools (T) and learning strategies (S) considered.}
\label{tab:Tools_strat}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{ID} & \textbf{Difficulty/Tool/Strategy}                                        & \textbf{ID} & \textbf{Difficulty/Tool/Strategy}                                       \\ \hline
P1          & Reading                                                    & T15         & Audio recording of lessons                                  \\
P2          & Writing                                                    & T16         & Video lessons                                               \\
P3          & Understanding difficult words                              & T17         & Supplementing study material with internet research         \\
P4          & Understanding the lessons                                  & S1          & A person reading for him/her                                \\
P5          & Concentration                                              & S2          & A map made by himself/herself                               \\
P6          & Paying attention during presential lessons                 & S3          & A scheme made by himself/herself                            \\
P7          & Paying attention during online lessons                     & S4          & A summary made by himself/herself                           \\
P8          & Memorising recently studied concepts                       & S5          & Repeat the studied material                                 \\
P9          & Remembering concepts studied during the exam               & S6          & Marking keywords                                            \\
P10         & Study time management                                      & S7          & Underlining with different colours                          \\
P11         & Taking notes                                               & S8          & Having a study group                                        \\
P12         & Limited time available to prepare a task/question/exam     & S9          & Having a tutor                                              \\
T1          & Human voice audio book                                     & S10         & Dyslexic student group to exchange resources                \\
T2          & Robotic voice audio book                                   & S11         & Presential lessons                                          \\
T3          & Different colour words                                     & S12         & Online lessons available                                    \\
T4          & Using the EasyReading font                                 & S13         & Taking breaks during lessons                                \\
T5          & Using a smart pen or tablet to take notes and record voice & S14         & Lesson slides available                                     \\
T6          & Clearer layout of the study material                       & S15         & Recording the lesson                                        \\
T7          & Having the key words of the text highlighted               & S16         & Taking notes                                                \\
T8          & Prepared concept maps                                      & S17         & Having the lesson plan in advance                           \\
T9          & Prepared schemes                                           & S18         & Dividing an examination/task/question into several parts    \\
T10         & Prepared summaries                                         & S19         & Only written tests                                          \\
T11         & E-Books                                                    & S20         & Only oral tests                                             \\
T12         & Digital tutor                                              & S21         & Conducting the exams in the presence of the professor alone \\
T13         & Images to help understand the meaning of difficult words   & S22         & Having an online database with notes made by other students \\
T14         & Images that help to memorise a concept                     &             &                                                             \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}


% Table 3
\begin{table}[H]
    \centering
\begin{tabular}{|c|c|c|}
\hline
    Case & $\alpha$ & $(1-\alpha)$ \\
    \hline
    \#1 & $2/3$ & $1/3$ \\
    \hline
    \#2  & $1/2$ & $1/2$ \\
    \hline
    \#3  & $1/3$ & $2/3$ \\
    \hline
    \#4  & $1/4$ & $3/4$ \\
    \hline
    \#5 & $1/5$ & $4/5$ \\
    \hline
    \#6 & $1/6$ & $5/6$ \\
    \hline
    \#7 & $1/7$ & $6/7$ \\
    \hline
    \#8 & $1/8$ & $7/8$ \\
    \hline
\end{tabular}
    \caption{Configuration of weights for the hybrid approach.}
    \label{tab:weights}
\end{table}


% Table 4
\begin{table}[h]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{similarity} & \textbf{n} & \textbf{MAE\_0} & \textbf{MAE\_1/8} & \textbf{MAE\_1/7} & \textbf{MAE\_1/6} & \textbf{MAE\_1/5} & \textbf{MAE\_1/4} & \textbf{MAE\_1/3} & \textbf{MAE\_1/2} & \textbf{MAE\_2/3} & \textbf{MAE\_1} \\ \hline
Euclidean           & 3                     & 1.1832          & 1.1315            & 1.1245            & 1.1152            & 1.1027            & 1.0846            & 1.0563            & 1.0049            & 0.9594            & 0.8920          \\ \hline
Euclidean           & 5                     & 1.1866          & 1.1347            & 1.1275            & 1.1179            & 1.1050            & 1.0863            & 1.0568            & 1.0015            & 0.9522            & 0.8750          \\ \hline
Euclidean           & 7                     & 1.1944          & 1.1412            & 1.1342            & 1.1250            & 1.1123            & 1.0939            & 1.0643            & 1.0085            & 0.9562            & 0.8735          \\ \hline
Euclidean           & 11                    & 1.2193          & 1.1650            & 1.1576            & 1.1479            & 1.1343            & 1.1146            & 1.0829            & 1.0244            & 0.9690            & 0.8782          \\ \hline
Cosine              & 3                     & 1.1839          & 1.1425            & 1.1371            & 1.1301            & 1.1212            & 1.1086            & 1.0895            & 1.0580            & 1.0309            & 0.9876          \\ \hline
Cosine              & 5                     & 1.2505          & 1.2020            & 1.1954            & 1.1867            & 1.1749            & 1.1576            & 1.1301            & 1.0815            & 1.0381            & 0.9647          \\ \hline
Cosine              & 7                     & 1.2754          & 1.2242            & 1.2177            & 1.2091            & 1.1972            & 1.1796            & 1.1511            & 1.0972            & 1.0486            & 0.9636          \\ \hline
Cosine              & 11                    & 1.3106          & 1.2550            & 1.2476            & 1.2380            & 1.2248            & 1.2054            & 1.1737            & 1.1136            & 1.0594            & 0.9659          \\ \hline
Pearson             & 3                     & 0.8217          & 0.8128            & 0.8118            & 0.8107            & 0.8096            & \cellcolor{yellow} \textbf{\large 0.8093}           & 0.8128            & 0.8314            & 0.8648            & 0.9661          \\ \hline
Pearson             & 5                     & 0.9092          & 0.8870            & 0.8843            & 0.8809            & 0.8766            & 0.8708            & 0.8639            & 0.8614            & 0.8735            & 0.9329          \\ \hline
Pearson             & 7                     & 0.9810          & 0.9494            & 0.9452            & 0.9398            & 0.9326            & 0.9227            & 0.9080            & 0.8913            & 0.8889            & 0.9222          \\ \hline
Pearson             & 11                    & 1.0868          & 1.0398            & 1.0336            & 1.0256            & 1.0147            & 0.9992            & 0.9756            & 0.9383            & 0.9160            & 0.9148          \\ \hline
\end{tabular}
\caption{Experimentation results considering the different similarity measures, number of neighbors and weights for the hybrid implementation. The best result (highlighted in the table) has been obtained by the hybrid method with an alpha value equals to 1/4, using Pearson as similarity measure and 3 neighbors.}
\label{tab:results}
\end{adjustbox}
\end{table}


% Table 5
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|}
        \hline
        \textbf{alpha} & \textbf{Best configuration} & \textbf{Best MAE}          \\ \hline
        0              & Pearson; n=3                & 0.8217                       \\ \hline
        1/8            & Pearson; n=3                & 0.8128                       \\ \hline
        1/7            & Pearson; n=3                & 0.8118                       \\ \hline
        1/6            & Pearson; n=3                & 0.8107                       \\ \hline
        1/5            & Pearson; n=3                & 0.8096                       \\ \hline
        \textbf{1/4}   & \textbf{Pearson; n=3 }      & \textbf{0.8093}              \\ \hline
        1/3            & Pearson; n=3                & 0.8128                       \\ \hline
        1/2            & Pearson; n=3                & 0.8313                       \\ \hline
        2/3            & Pearson; n=3                & 0.8648                       \\ \hline
        1              & Euclidean; n=7              & 0.8734                       \\ \hline
    \end{tabular}
\caption{Best configurations and MAEs obtained for the different weights in the hybrid model.}
\label{tab:weights_analysis}
\end{table}


% Table 6
\begin{table}[h]
\caption{Score received by dyslexic and non-dyslexic students that adopted or not the RS system suggestions}
\begin{tabular}{l|c|c|}
\cline{2-3}
 & \multicolumn{1}{l|}{Received RS suggestions} & \multicolumn{1}{l|}{Not received RS suggestions} \\ \hline
\multicolumn{1}{|l|}{Non-dyslexic} & 8.6 & 8.2 \\ \hline
\multicolumn{1}{|l|}{Dyslexic} & 8.2 & 7.1 \\ \hline
\end{tabular}
\label{table5}
\end{table}

